SheetSage2: Coherent Lead-Sheet Transcription with Synthetic Supervision

Transcribing music into a human-readable score requires a coherent understanding of rhythm, harmony, melody, and form. Two obstacles limit this goal: annotated recordings are scarce, and accurate local predictions can still produce inconsistent musical sequences. We present SheetSage2, a unified music transcription framework that combines synthetic data, task-specific structured decoding, and autoregressive distillation. Automatically annotated MIDI, rendered into audio, provides scalable supervision across music understanding tasks. Task-specific structured decoders integrate complementary musical cues and their temporal dependencies to produce musically coherent scores. Autoregressive distillation further retains transcription accuracy without task-specific dynamic programming at inference. Across eight benchmark collections, a single SheetSage2-AR model exceeds the listed prior systems on 12 of 15 benchmark--metric pairs in our evaluation, substantially improving over SheetSage1 and surpassing task-specific models on several benchmarks. Model weights and inference code are publicly available.

==> frontmatter.tex <==
\makeatletter
\newcommand{\submissionauthors}{%
  \icmlsetsymbol{equal}{*}
  \begin{icmlauthorlist}
    \icmlauthor{Junyan Jiang}{equal,nyu,mbzuai,ace,map}
    \icmlauthor{Ruibin Yuan}{equal,hkust,ace,map}
    \icmlauthor{Jiahao Pan}{hkust,map}
    \icmlauthor{Wei Xue}{hkust}
    \icmlauthor{Yike Guo}{hkust}
    \icmlauthor{Gus Xia}{mbzuai,nyu,map}
    \icmlauthor{Yann LeCun}{nyu}
  \end{icmlauthorlist}
  \icmlaffiliation{nyu}{New York University}
  \icmlaffiliation{mbzuai}{Mohamed bin Zayed University of Artificial Intelligence}
  \icmlaffiliation{ace}{ACE Studio}
  \icmlaffiliation{map}{Multimodal Art Projection}
  \icmlaffiliation{hkust}{The Hong Kong University of Science and Technology}
  \icmlcorrespondingauthor{Gus Xia}{gus.xia@mbzuai.ac.ae}
  \icmlcorrespondingauthor{Yann LeCun}{yann.lecun@nyu.edu}}
\newcommand{\mapicon}[1][1.6ex]{\raisebox{-0.15ex}{\includegraphics[height=#1]{assets/institutions/map.pdf}}}
\newcommand{\institutionentry}[3]{%
  \mbox{\textsuperscript{#1}\raisebox{-2pt}{#2}\hspace{3pt}#3}}
\newcommand{\techreportauthors}{%
  \begin{center}
    {\bfseries
      \mbox{Junyan Jiang\textsuperscript{1,2,3,\mapicon\,$*$}}\hspace{1.2em}%
      \mbox{Ruibin Yuan\textsuperscript{4,3,\mapicon\,$*$}}\hspace{1.2em}%
      \mbox{Jiahao Pan\textsuperscript{4,\mapicon}}\hspace{1.2em}%
      \mbox{Wei Xue\textsuperscript{4}}\\[3pt]%
      \mbox{Yike Guo\textsuperscript{4}}\hspace{1.2em}%
      \mbox{Gus Xia\textsuperscript{2,1,\mapicon\,$\dagger$}}\hspace{1.2em}%
      \mbox{Yann LeCun\textsuperscript{1\,$\dagger$}}\par}
    \vspace{6pt}%
    {\small%
      \institutionentry{}
        {\mapicon[9pt]}
        {Multimodal Art Projection}\hspace{1.2em}
      \institutionentry{1}
        {\includegraphics[height=6.5pt]{assets/institutions/nyu.pdf}}
        {New York University}\hspace{1.2em}
      \institutionentry{2}
        {\includegraphics[trim=140bp 205bp 650bp 185bp,clip,height=9pt]{assets/institutions/mbzuai.jpg}}
        {MBZUAI}\hspace{1.2em}
      \institutionentry{3}
        {{\setlength{\fboxsep}{1pt}\colorbox{black}{\includegraphics[height=7pt]{assets/institutions/ace-studio.png}}}}
        {ACE Studio}\\[2pt]
      \institutionentry{4}
        {\includegraphics[trim=0bp 0bp 525bp 0bp,clip,height=9pt]{assets/institutions/hkust.png}}
        {The Hong Kong University of Science and Technology}\par}
  \end{center}}
\newcommand{\techreportauthornotes}{%
  \global\icml@noticeprintedtrue
  {\let\thefootnote\relax\footnotetext{\raggedright\hspace*{-\footnotesep}%
    \textsuperscript{$*$}Equal contribution:
      Junyan Jiang \textless{}\href{mailto:junyan@acestudio.ai}{junyan@acestudio.ai}\textgreater{},
      Ruibin Yuan \textless{}\href{mailto:ruibiny@acestudio.ai}{ruibiny@acestudio.ai}\textgreater{}.
      \textsuperscript{$\dagger$}Corresponding authors:
      Gus Xia \textless{}\href{mailto:gus.xia@mbzuai.ac.ae}{gus.xia@mbzuai.ac.ae}\textgreater{},
      Yann LeCun \textless{}\href{mailto:yann.lecun@nyu.edu}{yann.lecun@nyu.edu}\textgreater{}.
    \ \\
    \Notice@String}}}
\makeatother

